IDSForge: Self-Explaining Network Intrusion Detection Through Neural Behavioral Rule Learning

Anomaly-based network intrusion detection systems (NIDS) can detect previously unseen attacks by identifying deviations from benign traffic. However, deep learning-based anomaly detectors typically rely on implicit decision boundaries, and post-hoc explanations may not faithfully reflect the detection logic. This makes alerts difficult to interpret and audit. To address this issue, we present IDSForge, an anomaly-based NIDS that directly learns explicit, executable behavioral rules from benign traffic, making its detection logic interpretable by design. IDSForge uses the same rule set for detection and explanation, ensuring explanation fidelity by construction. It uses an explicit distributional autoencoder trained only on benign samples to learn axis-aligned regions of benign traffic. A high-speed rule compiler then consolidates these instance-specific regions into a compact set of feature-level interval constraints. These rules can be executed directly by popular NIDS engines, supporting high-throughput inspection with low overhead. To adapt to changes in traffic, a self-distillation co-evolver updates the model and rule set incrementally when the false-positive rate on analyst-verified traffic exceeds a target threshold. Our evaluation shows that IDSForge reduces F1 error by $5.7\times$ to $47\times$ relative to state-of-the-art anomaly-based baselines. Deployed in Suricata, IDSForge sustains a throughput of 7.8 Gbps with a median per-packet latency overhead of 3.1 $\mu\text{s}$.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\noindent\textbf{Ante-hoc versus post-hoc interpretability.}
Post-hoc explainers are valuable for auditing existing black-box detectors~\cite{han2021deepaid,wei2023xnids,han2024rules}, but operators in high-stakes settings may find it difficult to act on explanations that disagree with detection decisions~\cite{rudin2019stop}. IDSForge treats interpretability as a design constraint. Its neural network serves as a \emph{rule generator} rather than the runtime detector. Neural computation is performed during offline training, while online detection uses range matching. A single rule base supports detection, explanation, auditing, and deployment. Operators can inspect, edit, or revoke individual rules without retraining the model.

\noindent\textbf{Adaptive adversaries.}
An attacker who knows the rule base may craft malicious flows that fall inside a benign hyper-rectangle. Proposition~\ref{prop:margin} shows that such evasion requires changing the violated features by at least the violation distance. Moreover, many flow features of attacks against Web services, such as the request rate of a flood or the number of failed logins in a brute-force attack, are linked to the attack's functionality. Constraining these features can therefore reduce attack effectiveness. Nevertheless, the rule base should be kept confidential, and features that are easy to manipulate (e.g., padding) can be excluded through the feature mask. Training-time poisoning and manipulation of false-positive feedback are separate threats. Since the adapter accepts only operator-confirmed false positives and bounds the growth of the acceptance region (Proposition~\ref{prop:forgetting}), poisoning requires compromising the triage process itself.

\noindent\textbf{Limitations.}
First, IDSForge uses flow-level statistical features and is subject to their limitations. For example, payload-level exploits within otherwise normal sessions may be statistically indistinguishable from benign flows and require complementary content inspection. Second, axis-aligned rules cannot compactly represent oblique correlations between features. This may increase the number of rules needed for highly correlated features. Feature-axis attention and rule reduction alleviate but do not eliminate this issue. Third, the adapter relies on operator feedback to identify false positives, and the trigger threshold $\theta_{\mathrm{FP}}$ controls the trade-off between update frequency and tolerance for false positives. Finally, our evaluation uses public datasets and a campus trace. Evaluating IDSForge on large-scale production Web traffic and offloading its rules to programmable switches~\cite{shi2025helios,li2024genos} remain directions for future work.

